WaferTrans: Enabling IOMMU-free Distributed Virtual Address Translation for Wafer-scale GPUs

Wafer-scale GPUs (WSGs) provide sufficient on-wafer bandwidth to make near-lossless Unified Memory feasible. However, existing designs still rely on a CPU-IOMMU to translate remote virtual-address accesses. This centralized mechanism scales poorly to tens of GPU dies: translation requests must traverse costly off-wafer hierarchies and contend for limited CPU-side resources, making address translation a critical bottleneck. We propose WaferTrans, an IOMMU-free distributed virtual-address translation design for WSGs. WaferTrans introduces PTE Presence Consistency (PTE-PC), a lightweight consistency model that tracks PTE insertions and removals, and equips each GPU with a PTE Presence Directory (PPD) that locates the GPU holding a requested PTE. It further employs a distributed PTE-PC mapping and a cooperative query mechanism to localize PTE-PC maintenance while preserving complete lookup coverage. Together, these mechanisms enable the GPU array to resolve remote translations within the wafer, eliminating its dependence on the CPU-IOMMU. Compared with the SOTA Trans-FW design, WaferTrans improves performance by 2.5x on average.

==> Makefile <==
# Build rules for the WaferTrans paper (MacTeX / TeX Live).

MAIN := main
PDF := $(MAIN).pdf
LATEXMK := latexmk
LATEXMK_FLAGS := -pdf -interaction=nonstopmode -file-line-error -halt-on-error

.PHONY: all pdf clean distclean help FORCE

all: $(PDF)

pdf: $(PDF)

$(PDF): FORCE $(MAIN).tex $(wildcard codes/*.tex) $(wildcard figures/*) refs.bib
	$(LATEXMK) $(LATEXMK_FLAGS) -g $(MAIN).tex
	$(LATEXMK) -c $(MAIN).tex
	$(RM) $(MAIN).bbl

FORCE:

clean:
	$(LATEXMK) -c $(MAIN).tex
	$(RM) $(MAIN).bbl

distclean:
	$(LATEXMK) -C $(MAIN).tex

help:
	@printf '%s\n' \
	  'make            Build main.pdf (default)' \
	  'make pdf        Build main.pdf' \
	  'make clean      Remove LaTeX temporary files' \
	  'make distclean  Remove temporary files and main.pdf'

